Social Bots for Online Public Health Interventions

According to the Center for Disease Control and Prevention, in the United States hundreds of thousands initiate smoking each year, and millions live with smoking-related dis- eases. Many tobacco users discuss their habits and preferences on social media. This work conceptualizes a framework for targeted health interventions to inform tobacco users about the consequences of tobacco use. We designed a Twitter bot named Notobot (short for No-Tobacco Bot) that leverages machine learning to identify users posting pro-tobacco tweets and select individualized interventions to address their interest in tobacco use. We searched the Twitter feed for tobacco-related keywords and phrases, and trained a convolutional neural network using over 4,000 tweets dichotomously manually labeled as either pro- tobacco or not pro-tobacco. This model achieves a 90% recall rate on the training set and 74% on test data. Users posting pro- tobacco tweets are matched with former smokers with similar interests who posted anti-tobacco tweets. Algorithmic matching, based on the power of peer influence, allows for the systematic delivery of personalized interventions based on real anti-tobacco tweets from former smokers. Experimental evaluation suggests that our system would perform well if deployed. This research offers opportunities for public health researchers to increase health awareness at scale. Future work entails deploying the fully operational Notobot system in a controlled experiment within a public health campaign.

==> src/equ.tex <==

\section{Machine Learning Models}


\subsection{Logistic Regression}
Logistic regression is a regression model that is used for binary classification. It was developed by David Cox in 1958 \cite{c36} and has been used in a wide variety of applications and fields. We implement a binary model that predicts the odds of a tweet being pro-tobacco based on the embedding of the tweet. Given a generalized linear model:
\begin{equation}
h_{\theta}(x)=\frac{1}{1+e^-\theta^{T}x}
\end{equation}
The probability that a tweet is pro-tobacco or not pro-tobacco is modeled as: \begin{equation}
Pr(y|x;\theta)=h_{\theta}(x)^{y}(1-h_{\theta}(x))^{(1-y)}
\end{equation}
Which we then maximize the log likelihood using a gradient descent algorithm.
\begin{equation}
log L (\theta|x)=\sum_{i=1}^{N}log Pr(y_{i}|x_{i};\theta)
\end{equation}
Our implementation used the LogisticRegressor in the TensorFlow module \cite{c37}. 


\subsection{Decision Tree}
Decision Trees are another classification method which are based on an underlying probability model \cite{c38}. Given the manually labeled data which consist of $y$, the label and $\vec{x}$, the embedding of the tweet, the data can be viewed as $(x_{1},x_{2},...x_{p},y)$ where each $x_{i}$ is a feature of the embedding. We applied the classification algorithm proposed in \cite{c39}. Working from the top and going down the tree, the Gini impurity which is a measure of how to best split the features is defined as:
\begin{equation}
I_{G}(p)=\sum_{i=1}^{K}p_{i}\sum_{i\ne j}p_{j} ; \sum_{i\ne j}p_{j}=1-p_{i}
\end{equation}


\subsection{Support Vector Machines}

Support Vector Machines were first theorized in 1963 \cite{c35} in and implementation algorithms used in this paper is from 1993 \cite{c34} . Given $n$ data points of the form $(\vec{x}_{1},y_{1})...(\vec{x}_{n},y_{n})$ where $\vec{x}_{i}$ is a $p$ dimensional vector that is the embedding of a tweet. Furthermore, $\vec{y}_{i}$ is either 1 for pro-tobacco tweet or -1 for non pro-tobacco tweet. 
SVM is a method to do a binary classification by developing a hyperplane $\vec{w}\cdot\vec{x}-b=0$ where $\vec{w}$ is the normal vector of the hyperplane and $b$ is a measure of the offset.  
In the non-linear implementation of soft-margin, the hinge loss function is shown in Equation 2 which is minimized using a sub-gradient descent algorithm. 
The $\lambda$ is a parameter that captures the trade off between margin-size and ensuring $\vec{x}_{i}$ in on the correct side of the margin. 
\begin{equation}
[\frac{1}{n} \sum_{i=1}^{n} max ( 0, 1-\vec{y}_{i}(\vec{w}\cdot\vec{x}_{i}-b))]+\lambda||\vec{w}||^{2}
\end{equation}

\subsection{Multi-Layer Perceptrons}
Multi-Layer Perceptrons (MLP) is standard neural network in artificial intelligence that is trained using backpropagation. Other than the nodes in the input layer, the other nodes use a nonlinear activation function. Here we apply a simple MLP which only has one hidden layer \cite{c40}. In this analysis, we used the rectified linear unit (ReLU) activation function defined by \cite{c41}:
\begin{equation}
f(x)=x^{+}=max(0,x)
\end{equation} 

\subsection{Char-CNN}
Character-based convolutional neural networks (Char-CNN) treat text as a raw signal at the character level\cite{c20}. This leverages the temporal convolutional module:
\begin{equation}
h(y)=\sum_{x=1}^{k}f(x)\cdot g(y\cdot d-x+c)
\end{equation}
where $g(x)$ is a discrete input function and $f(x)$ is a discrete kernel function. The stride of the convolution $h(y)$ between $f(x)$ and $g(x)$ is $d$ and $c$ is an offset constant \cite{c20}. The Char-CNN was implemented using the TensorFlow module as well \cite{c37}. 


\begin{figure*}
  \includegraphics[width=\textwidth,height=4cm]{images/complete.png}
  \caption{Overall Notobot system}
  \label{fig:complete}
\end{figure*}


==> src/pseudo.tex <==
\begin{algorithm}
\caption{NoBotCo}
\begin{algorithmic} 
%\REQUIRE Consumer Key \& Secret
%\REQUIRE Assess Token \& Secret 
%\ENSURE Network Connectivity
\WHILE{NoBotCo Active}
\STATE current\_id='' \# set current\_id null
\STATE \textbf{Search\_Tobacco\_Tweets}
\STATE count=1 \#process one at a time
\STATE result\_type='recent'
\STATE lang='en' \#English only
\STATE since\_id='current\_id' \#next posted tweet
\IF{Tweet Found}
\STATE \textbf{Pro-Tobacco\_Classifier}
\IF{tweet\_text=pro-tobacco}
\STATE \textbf{Select\_Intervention\_Tweet}
\STATE \textbf{Post\_Intervention\_Tweet}
\STATE current\_id=since\_id
\ELSE
\STATE current\_id=since\_id
\ENDIF
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}
